Minimally Intrusive Access Management to Content Delivery Networks based on Performance Models and Access Patterns

This paper presents an approach to managing access to Content Delivery Networks (CDNs), focusing on combating the misuse of tokens through performance analysis and statistical access patterns. In particular, we explore the impact of token sharing on the content delivery infrastructure, proposing the definition of acceptable request limits to detect and block abnormal accesses. Additionally, we introduce countermeasures against piracy, such as degrading the quality of service for pirate users to discourage them from illegal sharing, and using queuing models to quantify system performance in different piracy scenarios. Adopting these measures can improve the consistency and efficiency of CDN access and cost management, protecting the infrastructure and the legitimate user experience.

==> name.tex <==
https://github.com/xiumulty/CVE/blob/main/Lead%20management%20system%20v1.0/sql%20in%20changePassword.php.md
https://github.com/ARMmbed/mbedtls/releases/tag/v3.1.0
https://github.com/convos-chat/convos/commit/86b2193de375005ba71d9dd53843562c6ac1847c
https://github.com/pcmacdon/jsish/issues/52 

==> old_outdated/name.tex <==
https://github.com/xiumulty/CVE/blob/main/Lead%20management%20system%20v1.0/sql%20in%20changePassword.php.md
https://github.com/ARMmbed/mbedtls/releases/tag/v3.1.0
https://github.com/convos-chat/convos/commit/86b2193de375005ba71d9dd53843562c6ac1847c
https://github.com/pcmacdon/jsish/issues/52 
